GRAPHSHAP: Explaining Identity-Aware Graph Classifiers Through the Language of Motifs

Most methods for explaining black-box classifiers (e.g. on tabular data, images, or time series) rely on measuring the impact that removing/perturbing features has on the model output. This forces the explanation language to match the classifier's feature space. However, when dealing with graph data, in which the basic features correspond to the edges describing the graph structure, this matching between features space and explanation language might not be appropriate. Decoupling the feature space (edges) from a desired high-level explanation language (such as motifs) is thus a major challenge towards developing actionable explanations for graph classification tasks. In this paper we introduce GRAPHSHAP, a Shapley-based approach able to provide motif-based explanations for identity-aware graph classifiers, assuming no knowledge whatsoever about the model or its training data: the only requirement is that the classifier can be queried as a black-box at will. For the sake of computational efficiency we explore a progressive approximation strategy and show how a simple kernel can efficiently approximate explanation scores, thus allowing GRAPHSHAP to scale on scenarios with a large explanation space (i.e. large number of motifs). We showcase GRAPHSHAP on a real-world brain-network dataset consisting of patients affected by Autism Spectrum Disorder and a control group. Our experiments highlight how the classification provided by a black-box model can be effectively explained by few connectomics patterns.

==> 9_dump.tex <==
\section{Appendix}
\label{sec:dump}

\begin{comment}
All code is available at \href{https://anonymous.4open.science/r/LOG_GraphSHAP-26B5/}{this anonymised repository.}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Extended Intro}

Model interpretability of prediction tasks is increasingly needed for accountability, trust, fairness and debugging~\cite{shneiderman2020human,gilpin2018explaining,bhatt2020explainable,panigutti2020fairlens}, especially when machine learning algorithms are incorporated into decision-making that may directly affect people’s lives~\cite{tan2018distill}. While transparent-by-design models should be preferred for high stakes decisions \cite{rudin2019stop}, in an increasing number of cases black-boxes are already deployed and used as decision support-systems. Therefore, researchers in AI-intensive companies and academia devised model-agnostic techniques to provide local post-hoc explanations on model predictions~\cite{guidotti2018survey,gilpin2018explaining}. While such methods mainly focus on tabular data~\cite{ribeiro2016should,lundberg2017unified}, and have been further extended to images~\cite{selvaraju2017grad,shrikumar2017learning} and time series~\cite{assaf2019explainable}, much less attention have been devoted to provide actionable explanations for graph classification tasks.

Graphs are a powerful mathematical representation of several real-world systems and, as learning from networked-structures requires ad-hoc approaches~\cite{zhou2020graph,zhang2019graph}, so do explanation techniques aimed at interpreting algorithmic decisions on graphs.
Most model-agnostic explainability methods either rely on tabular data or on some form of vectorisation of the original input space: explanations are then provided by ranking the input features according to some scores~\cite{ribeiro2016should,lundberg2017unified,chen2018learning}, thus \emph{constraining the explanations to be expressed in the very same language of the training data of the black-box}.
Following the same approach in a graph classification task, one could embed the adjacency matrix of a graph in a $d$-dimensional space vector, and then feed the resulting graph dataset to a learning algorithm.
When applying standard explainability methods, the explanation language for one given graph would correspond either to the whole adjacency matrix, or to the $d$-dimensional vector.
The former option contains a high number of fine-grain features, while the latter option has limited explainability due to the not interpretable embedding transformation. Neither option is well suited for human understanding and interpretation.

Here we argue that $(i)$ a good explanation method for graph classification should be fully agnostic w.r.t. the internal representation used by the black-box; and $(ii)$ a good explanation language for graph classification tasks should be represented by motifs, as they are higher order structures
which encode more information and are more adequate for human understanding. Thus our approach completely decouples the input space of the classifier from the explanation space.


\subsection{Overview of contributions and roadmap}
With the growing availability of Graph Neural Networks (GNNs) methods which can indifferently handle several different predictive tasks, such as, e.g., link predictions \cite{cai2020multi,zhang2018link}, node classification~\cite{henaff2015deep,liu2020towards,gao2019graph}, and classification of the whole graph~\cite{zhang2018end,xu2018powerful}, the term \emph{``graph classification''} is more and more used in the literature to indicate a general class of machine learning tasks on graph-structured data, typically having additional information in the form of nodes and edges features. In this paper, instead,  we consider a specific type of graph classification that arises in many application domains, in which a specific node id corresponds to the same entity in all the input networks: for instance, in classification of brain networks, the same node id represents the same brain region in all the input graphs.
 We call this setting graph classification \emph{with node identity awareness} \cite{gutierrez2019embedding,lancianokdd,AbrateB21}. While not every application domain requires node identity awareness, it is crucial to exploit these property whenever it occurs, as ignoring it represents an important loss of information.

More formally, we are given a database $\mathcal{D}$ of graphs, where each graph $G  \in \mathcal{D}$ is defined over the same set of nodes $\mathcal{V}$ and it has a label in $\{0,1\}$ (for sake of simplicity we consider the binary classification case, but our approach can be easily extended to te multi-class case). Let $\mathcal{G}$ denote the set of all possible graphs defined over $\mathcal{V}$, we want to learn a model that for any unseen graph $G \in  \mathcal{G}$  it is able to predict whether it belongs to class 0 or 1.

In this context of graph classification with node identity awareness, we are given a ``black-box'' model $B: \mathcal{G} \to [0,1]$ returning, for any graph $G \in \mathcal{G}$, the probability that $G$ is in class 1.
Here ``black-box'' means we can not inspect $B$, we do not know the learning algorithm that produced $B$, nor its parameters, nor we have access to its training data. $B$ might as well be an opaque executable or an exposed API. The only requirement about $B$ is that it can be queried at will. The problem tackled in this paper is that of  producing an explanation for the black-box graph classifier logic, using an explanation language (motifs) that does not coincide with the input space of the classifier (adjacency matrix).

After providing the needed background (\S \ref{sec:rw}) we formally state our problem (\S \ref{sec:problem_statement}), and we introduce our method \method (\S \ref{sec:pipeline}), a Shapley-based approach for motif-based explanations of black-box graph classifiers.
One key mechanism in any Shapley-based explanation approach is the creation of the features coalitions to query the black-box. In our setting this corresponds to the task of masking a set of motifs from a given graph. For this basic task we propose three different approaches (\S \ref{sec:motif_masking}).

The explanation language (i.e. a set of motifs) is assumed to be given in input. This can be provided by the domain expert or mined from a dataset (when available). When the input set of motifs is too large, the exact estimation of Shapley values becomes computationally not doable. For dealing with these cases, we propose a simple approximation kernel (\S \ref{sec:kernel}).

As a (non-trivial) side contribution we devise a synthetic dataset generator for graph classification (\S \ref{sec:sythentic_data_generation}) which we use to benchmark \method (\S \ref{sec:gs_on_synthetic_data}),
to empirically compare different masking approaches (\S \ref{sec:masking_experiments}),
and to demonstrate that the proposed kernel is able to approximate the exact Shapley values with a computational complexity that is linear with respect to the number of explained features (\S \ref{sec:kernel_experiments}). We also develop a algorithms for motifs mining and ranking (\S \ref{sec:mining}) and a custom graph convolutional layer able to deal with a graph dataset with node identity (\S \ref{sec:gconv}).

Finally, we test \method on a real-world brain-network dataset consisting of patients affected by Autism Spectrum Disorder and a control group. Our experiments highlight how the classification provided by a black-box model can be effectively explained by few connectomics patterns (\S \ref{sec:brain}).
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{Synthetic Dataset Generation Algorithm}
\label{sec:synth_algo}

\DontPrintSemicolon
\begin{algorithm}[h!]
 \KwIn{$n$: number of nodes,
 $n_g$: number of graphs, \newline
 $d_g$: graph density , \newline
 $\mathcal{M}$: set of $n_m$ motifs, \newline
 $\rho(k), \forall k \in [n_m]$: motif probabilities,
 \newline
 $\mathbf{C} \in [0,1]^{n_m \times n_m}$: motif correlation matrix  }
 \KwResult{Labelled graph dataset $(\mathcal{G},\tau)$}
$\mathcal{G} \leftarrow \emptyset$\;
Initialize $\mathbf{R} \in [0,1]^{n_g \times n_m} $ with random values \;
\For{$j$ in $0 .. n_g-1$}{ \label{synth:line:for}
$G \leftarrow \mathrm{ER}(\mathcal{V} = \{1..n\}, d_g)$\;
\For{$k$ in $0 .. n_m-1$}{

\If{$\mathbf{C}_{k} \cdot \mathbf{R}_{j}^\intercal \leq \rho(k)$}{
\eIf{$(j\mod 2) \equiv (k\mod 2)$}{
add edges of motif $\mathcal{M}_k$ to $G$
}{
remove edges of motif $\mathcal{M}_k$ from $G$
}
}
}%end for
$\tau(G) \leftarrow j\mod 2$\;
$\mathcal{G} \leftarrow \mathcal{G} \cup \{G\}$\;
}
\Return $(\mathcal{G},\tau)$
\caption{Synthetic Graphs Generation}
\label{algo:synth}
\end{algorithm}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Synthetic dataset validation}
\label{sec:sythentic_data_validation}

To validate the synthetic graph generation we test class separability for different configurations.
In particular we generate datasets  with 100 graphs per class, number of nodes $n = |\mathcal{V}|=100$, graph density $0.2$, and a range of parameter configurations regarding motif number and size and perturbation probability. For these experiments we did not enforce any kind of correlation within motifs (referring to the notation in~\ref{algo:synth}, $\mathbf{C}$ is an identity matrix).

Class separability is measured as the two-sample Kolmogorov–Smirnov test on the distributions of intra- and inter-class distances, where we use the Jaccard distance $J(G_i,G_j)$ for intra-class ($\tau(G_i)=\tau(G_j)$)  and inter-class ($\tau(G_i)\neq\tau(G_j)$) distances.
For each parameter setting we repeat the experiments 30 times, obtaining the results shown in Figure~\ref{fig:synth_separability}: each curve corresponds to a different configuration, with the solid line representing the average result and the shadow area the error range.

\begin{figure}[h]%b!
 %\vspace{-2mm}
  \centering
    \includegraphics[width=0.45\textwidth]{_figs/synthgen_separability.pdf}
     %\vspace{-6mm}
    \caption{Class separability on different synthetic graphs.}
    \label{fig:synth_separability}
     %\vspace{-2mm}
\end{figure}

% \FloatBarrier

As expected, for all configurations higher perturbation probability induces higher class separability. Moreover, class separability is larger for larger number of injected motifs and larger size of these motifs (expressed as number of edges).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{Approximation Kernel Visualized}

\begin{figure}[h]
  \centering
    \includegraphics[width=0.45\textwidth]{_figs/graphshap_lattice_2.pdf}.
    \caption{Shapley lattice and depth of layers for the case of 5 input features to explain. The number of nodes in the lattice grows exponentially with the number of input features, while the number of layers grows linearly.}
    \label{fig:lattice_kernel}
\end{figure}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Motif mining and ranking}
\label{sec:mining}

We envision \method as a tool for discovering the importance of candidate subgraphs in a graph classification ML task. Ideally, these subgraphs might be provided from domain experts or inferred from domain-specific literature. However, it might also be interesting to automatically generate potential subgraph candidates, so that \method can compute explanation scores for previously unexplored motifs.

In order to do so, we developed custom algorithms for mining motifs from a graph dataset and selecting a subset through ranking. Despite the task not being novel, we preferred to develop a novel algorithm for practical reasons. First of all, many subgraph mining algorithms are based on computationally-intensive procedures of subgraph- and graph isomorphism~\cite{gspan}, but the node identity property makes these steps unnecessary, as they can be replaced by the much easier task of matching node IDs. Another family of well-established similar algorithms is frequent-itemset mining~\cite{frequent-itemset}. However, we are interested in mining motifs, which are connected subsets of edges, and frequent-itemset mining algorithms do not check for connectivity. One option could be use these algorithms to mine edge subsets and then filter them in order to keep only the subsets corresponding to motifs, but this is a clearly disadvantageous approach, as it temporarily produces a large amount of candidates that will be subsequently filtered out. Finally, we wanted to develop our algorithm in Python, so that it could be used within the \method suite more naturally.

\DontPrintSemicolon
\begin{algorithm}[h!]
 \KwIn{$\mathcal{G}$: set of graphs defined over nodes $V$, $s$: support threshold}
 \KwResult{$\mathcal{M}$: set of motifs with support $s$ over $\mathcal{G}$}
$\mathcal{E} \leftarrow \{e \equiv (v_i,v_j) : \{v_i,v_j\} \subseteq V, supp(e,\mathcal{G})\geq s \}$\;
$\mathcal{T} \leftarrow \{\{e_1,e_2\} : \{e_1,e_2\} \subseteq \mathcal{E}, connected(e_1,e_2),supp((e_1,e_2),\mathcal{G})\geq s \}$\;
$\mathcal{M}$ $\leftarrow$ $\mathcal{T}$\;
\For{goal $\leftarrow$ 3 \KwTo$ \left|V\right|$}{
\ForEach{$m \in \mathcal{M}$, $t \in \mathcal{T}$}{
\If {$\left| m \cup t \right| \equiv$ goal and supp($m \cup t,\mathcal{G})$ $\geq s$}{
$\mathcal{M}$ $\leftarrow$ $\mathcal{M} \cup t$\;
}
}
}
\Return $\mathcal{M}$
\caption{Motif Mining}
\label{algo:mining}
\end{algorithm}

 We therefore developed a custom motif mining algorithm, whose high-level pseudocode is described in Algorithm~\ref{algo:mining}). We rely on the concept of {\em support}, and exploit the function $supp(m,\mathcal{G})$ to indicate the number of graphs in $\mathcal{G}$ that $m$ is a subgraph of.
 We use {\em twoplets} (two-edges motifs) as building blocks and we iteratively build increasingly bigger motifs, as long as their support over the dataset is above a given threshold.

 Once a set of motifs is mined, our aim is to extract motifs which are promising for their discriminative potential, for being particularly frequent in one class and not-so-frequent in the other class. More in details, given a mined set of motifs $\mathcal{M}$, we select a subset of motifs according to a greedy ranking-and-filtering procedure. Given our labelled graph dataset $\mathcal{G}$, let $\mathcal{G}_0$ and $\mathcal{G}_1$ be the two sets of graphs in $\mathcal{G}$ with label 0 and 1 respectively. For each motif $m_i \in \mathcal{M}$ we can compute the support over the two sets $\mathcal{G}_0$ and $\mathcal{G}_1$ combine these two values values to compute a {\em cross-support} score $CS$:
$$CS_i = abs(log_2(\frac{supp(m_i,\mathcal{G}_0)+1}{supp(m_i,\mathcal{G}_1)+1}))$$
We use the $CS$ score to rank the motifs and greedily select those having a size over a minimum number of edges and a  Jaccard distance of edges from the already selected motifs larger than a given threshold. The process is summarized in is described in Algorithm~\ref{algo:ranking}.

 \DontPrintSemicolon
\begin{algorithm}[h!]
 \KwIn{$\mathcal{G}$: set of graphs, $\mathcal{M}$: set of motifs, $dt$: distance threshold, $st$: size threshold, $k$: output size}
 \KwResult{$\hat{\mathcal{M}}$: selected motifs}
Compute $CS_i$ for all $m_i \in
\mathcal{M}$\;
Rank $\mathcal{M}$ for decreasing $CS$-score\;
$\hat{\mathcal{M}} \leftarrow \emptyset$\;
\While{$\left| \hat{\mathcal{M}} \right| \leq k$ and $\left| \mathcal{M} \right| > 0$}{
$m_i \leftarrow pop(\mathcal{M})$\;
$mindist \leftarrow min(\{Jaccard(m_i,m_j) \ \forall m_j \in \hat{\mathcal{M}}\})$\;
\If{$mindist \geq dt$ and $\left|m_i\right| \geq st$ }{$\hat{\mathcal{M}} \leftarrow \hat{\mathcal{M}} \cup \{m_i\}$}
}

\Return $\hat{\mathcal{M}}$
\caption{Motif Ranking}
\label{algo:ranking}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}


\subsection{Graph Convolution with node identity}
\label{sec:gconv}

Despite not being the focus of this paper, an efficient black-box for graph classification is needed to validate \method, with graph convolutional neural networks being our method of choice. Several existing frameworks and libraries allow to create and train such models, but -- to the best of our knowledge -- there is no Python-based library for graph convolutional layers able to exploit the node identity property. Without node identity, all nodes in different graphs have to be considered as different entities, and therefore when dealing with batches of graph data-points, their adjacency matrices have to be composed as shown in Figure~\ref{fig:stack_adjm}~(left). This operation requires to align all adjacency matrices along the diagonal of a batch-adjacency matrix which is created on the fly, and renaming all nodes in all graphs so that the same ID are not reused. Conversely, in the node identity setting, all adjacency matrices of different graphs share the same shape, and nodes with the same ID represent the same entity across all graphs. In short, the correct way to represent a batch of graph data-points is to stack the single adjacency matrices along a third axis.%, as shown in Figure~\ref{fig:stack_adjm}~(right).

%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.6\textwidth]{_figs/stack.pdf}.%pdf}
%    \caption{Composition of a batch of adjacency matrices in the case of a graph convolution without node identity (left) and in the case of a graph convolution with node identity (right).}
%    \vspace{-0.3cm}
%    \label{fig:stack_adjm}
%\end{figure}

We therefore used a custom graph convolution layer for the node identity setting; its implementation is as follows:

 \begin{verbatim}
 class GConvNodeID(tf.keras.layers.Layer):
     def __init__(self,num_feat,num_out,activation):
         super(GConvNodeID,self).__init__()
         self.W = tf.Variable(GlorotUniform(seed=None)(shape=(num_feat,num_out)))
         self.activation = activation
     def call(self,A,X):
         XW = tf.einsum('bij,jk->bik',X,self.W)
         AXW = tf.einsum('bij,bjk->bik',A,XW)
         return self.activation(AXW)
 \end{verbatim}
 The $call()$ method implements, in batch mode, the definition of a standard graph convolution:
$$\mathbf{X}^{\prime} = \mathbf{\hat{D}}^{-1/2} \mathbf{\hat{A}}
\mathbf{\hat{D}}^{-1/2} \mathbf{X} \mathbf{W}$$

where $\mathbf{\hat{A}} = \mathbf{A} + \mathbf{I}$ denotes the adjacency matrix with inserted self-loops and $\mathbf{\hat{D}}_{ii} = \sum_{j=0} \mathbf{\hat{A}}_{ij}$ its diagonal degree matrix.


This graph convolution layer is used as a building block in the graph convolutional neural network that we used as a  black-box throughout all the experiments described in the following section. The final architecture is inspired on the Deep Graph CNN model proposed in~\cite{zhang2018end}:
the input graphs with node identity are first passed through multiple graph convolution
layers where node information is propagated between neighbors.
The SortPooling layer is replaced by a conventional concatenation layer, in order to keep the node identities, and then passed to traditional CNN structures to learn a predictive model.

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{Detailed brain-motif visualization}
\begin{figure}[h]
  \centering
    \includegraphics[width=0.45\textwidth]{_figs/braaaainz.pdf}.
    \caption{Expanded visualization of the motifs $M_1$, $M_2$, $M_5$, $M_8$ described in the paper}
    \label{fig:braainz}
\end{figure} 
\end{comment}
